Correlation Propagation Networks for Scene Text Detection

In this work, we propose a novel hybrid method for scene text detection namely Correlation Propagation Network (CPN). It is an end-to-end trainable framework engined by advanced Convolutional Neural Networks. Our CPN predicts text objects according to both top-down observations and the bottom-up cues. Multiple candidate boxes are assembled by a spatial communication mechanism call Correlation Propagation (CP). The extracted spatial features by CNN are regarded as node features in a latticed graph and Correlation Propagation algorithm runs distributively on each node to update the hypothesis of corresponding object centers. The CP process can flexibly handle scale-varying and rotated text objects without using predefined bounding box templates. Benefit from its distributive nature, CPN is computationally efficient and enjoys a high level of parallelism. Moreover, we introduce deformable convolution to the backbone network to enhance the adaptability to long texts. The evaluation on public benchmarks shows that the proposed method achieves state-of-art performance, and it significantly outperforms the existing methods for handling multi-scale and multi-oriented text objects with much lower computation cost.

==> analysis.tex <==
\section{Analysis of Markov Clustering Network}

\subsubsection{Detection Model}
Markov Clustering Network (MCN) \cite{liu2018clustering} is an object detection method based on graph clustering. As shown in Figure \ref{fig:method}, a latticed stochastic flow graph $G(V,E)$ \cite{van2001graph} with $\frac{H}{U}\times\frac{W}{U}$ nodes is constructed by MCN from an input image with size of $H\times W$. The nodes $V$ in $G$ correspond to the feature vectors extracted from the overlapping regions of the image, and the edges $E$ are weighted by the flow values $f_0$, $f_1$, $f_2$ and $f_3$ predicted by MCN. The presence of an object is jointly represented by nodes with strong connections to each other, and the background region is represented by isolated nodes. The objectness is implicit in the flow values and can be extracted by Markov Clustering. \par

\begin{figure}[]
	\centering
	\includegraphics[width=0.5\linewidth]{figures/method.pdf}
	\caption{Markov Clustering Network.}
	\label{fig:method}
\end{figure}

\subsubsection{Markov Clustering} 
Markov Clustering \cite{van2001graph} is an algorithm to identify the strongly connected nodes in a weighted graph and group them into clusters according to their local connections. In MCN, Markov Clustering is applied to recognize instance-level object regions. In Markov Clustering, a flow matrix $M_0$ is constructed from $G$ with entry $M_0(m,n)$ representing the flow value from node $V(i_n,j_n)$ to node $V(i_m,j_m)$ \footnote{We use both 1D and 2D notation, alternatively, to index a node. The transformation between 1D notation $m$ and 2D notation $(i_m,j_m)$ can be represented by $m = i_m + \frac{H}{U}\cdot j_m$.}. It consists of a set of iterations including matrix-matrix multiplication and non-linear transformation, which are illustrated in Algorithm \ref{alg:mc},
\begin{algorithm}
	\caption{Markov Clustering}
	\label{alg:mc}
	\begin{algorithmic}[1]
		\State {\textbf{Initialize}:}
		$t=0$\;
		\While{$t < N$} 
		\State{$M_t = M_{t-1}\cdot M_0$\;} // expand 
		\State{$M_t(m,n) = \frac{M_t(m,n)}{\sum_l{M_t(l,n)}}$}\; // inflate
		\State{$M_t(m,n) = 0,\ if \ M_t(m,n) < \emph{threshold}$}\; // prune
		\EndWhile
		\State {\textbf{Output}: $M_N$ as a clustering.}
	\end{algorithmic}
\end{algorithm}
where $M_t$ is the intermediate result at $t$-th iteration and $N$ is the number of iterations for convergence. The columns of $M_t$ corresponding to the same cluster will converge to the same one-hot vector. It is reflected on $G$ that nodes within a strongly connected group will flow to the same attractor node at the end, which helps to identify any potential cluster. \par

\subsubsection{Forward Complexity} As illustrated in Algorithm \ref{alg:mc}, the computation of MC is dominated by the matrix-matrix multiplication in the expansion step. The complexity of expansion is $O(N(HW)^3/U^6)$, which is mainly decided by the graph size and number of MC iterations. In fact, there exist large amount of redundancy in Markov Clustering. Since MCN predicts a graph that only has four directed edges for each node, the flow matrix $M_0$ is highly sparse. For a $512\times 512$ image with upsampling factor $U = 16$, more than XX$\%$ computation are wasted.  

\subsubsection{Probability Interpretation}
From the probability perspective, the stochastic flow graph (SFG) is modeling the Markov random walk process, and the flow values at each node describe the corresponding transition probability. These transition probabilities are recorded in the columns of flow matrix $M_0$. The $n$-th column $M_0(:,n) \in \mathbb{R}^{\frac{H}{U}\cdot\frac{W}{U}}$ of $M_0$ is representing the transition distribution $P_0(V|V(i_n,j_n))$ of a Markov random walk starting at node $V_n$. For each node $V(i,j)$, there exists a stationary distribution $P(V|V(i,j))$ describing possible attractor node of this process. A cluster is denoted as a set of strongly connected node share the same attractor that has highest probability in $P(V|V(i,j))$. Markov Clustering is actually computing the stationary distribution $P(V|V(i,j))$ for each node. The $n$-th column of converged flow matrix $M_N(:,n)$ represents the stationary distribution for node $V(i_n,j_n)$.

\subsubsection{Learning}
The learning process of MCN can be treated as minimizing the mean cross-entropy loss of each node between predicted stationary distribution and ground-truth distribution \cite{liu2018clustering}. The end-to-end training is enabled by the differentiability of Markov Clustering. The Markov Clustering outputs the stationary distribution $M_N(:,m) \in \mathbb{R}^{\frac{H}{U}\cdot\frac{W}{U}}$ of potential attractors for each node. The ground-true label for each node is defined as the target distribution $y_f(i_m,j_m) \in \mathbb{R}^{\frac{H}{U}\cdot\frac{W}{U}}$. Given the converged flow distribution $M_N$ and the target distribution $y_f$ for all nodes, the loss function is represented by:
\begin{align}
\begin{split} &C_f = \frac{1}{H/U\cdot W/U}\sum_{i_m}\sum_{j_m} L_f(i_m, j_m), \end{split} \\
\begin{split} &L_f(i_m, j_m) = -y_f(i_m, j_m)\cdot \ln(M_N(:,m)). \end{split} 
\end{align}
The operations of Markov Clustering is visualized as the computing graph shown in Figure \ref{fig:flow_grad}, and the corresponding gradients of $C_f$ respecting to predicted $M_0$ is represented by Equation \ref{eq:flow_grad}-\ref{eq:flow_grad_2}.

\begin{figure}[]
	\centering
	\includegraphics[width=0.7\linewidth]{figures/flow_grad.pdf}
	\caption{Computing graph of Markov Clustering. It takes initial flow matrix $M_0$ as input and outputs a converged flow $M_N^P$ to compute $C_f(M_0)$.}
	\label{fig:flow_grad}
\end{figure}

\begin{align}
\label{eq:flow_grad}
\begin{split} &g_{M_N^P} = \partial{C_f}/\partial{M_N^P}, \end{split} \\ 
\begin{split} &g_{M_t^I} = g_{M_t^P}\cdot f'_P(M_t^I),  \end{split} \\
\begin{split} &g_{M_t} = g_{M_t^I}\cdot f'_I(M_t),  \end{split} \\
\begin{split} &g_{M_{t-1}^P} = M_0^T\cdot g_{M_t},  \end{split} \\
\begin{split} &g_{M_0}(t) = g_{M_t}\cdot (M_{t-1}^P)^T,  \end{split} \\
\begin{split} &g_{M_0} = \partial{C_f}/\partial{M_0} = g_{M_0^P} + \sum_{i=1}^N{g_{M_0}(i)}, \end{split} \label{eq:flow_grad_1} \\
\begin{split} &f'_P(x) = 1\ if\ x > 0,\ else\ 0, \end{split} \\
\label{eq:flow_grad_2}
\begin{split} &f'_I(x) = 1. \end{split}
\end{align}

\subsubsection{Backward Complexity} ...

The complexity of MC gradient computation is $O(2N(HW)^3/U^6)$, which has the same order as that of forward pass. Naively implementation of Markov Clustering without considering the topology of stochastic flow graph brings large amounts of wastes in computation and storage.

\emph{runtime and memory footprint v.s. graph size}

\emph{runtime and memory footprint v.s. average number of node in a bbox}

\emph{runtime v.s. number of MC iterations}

\subsubsection{Performance Coupling} ...

The detection accuracy depends on the number of MC iteration $N$, because accurate the stationary probability relies on sufficient iterations for convergence. When an object region is large, insufficient iteration can result in split of a bounding box which reduce the performance. $N$ is a task-specific parameter and varies in different scenarios. On the other hand, number of MC iterations is also different for different clusters. 
\emph{accuracy v.s. number of MC iterations}

\subsubsection{Sparse Flow Matrix}  ...

\emph{Sparsity of Flow Matrix}





==> details.tex <==
\section{Implementation Details}

The architecture of CPN, inference flow and training flow are illustrated in Fig. \ref{fig:sys_flow}. An CPN consists of a CNN backbone network. All the fully-connected layers are removed, resulting in an output resolution of $1/16$. Here we apply VGG-16 \cite{simonyan2014very} and ResNet-50 \cite{he2016deep} independently and the performance comparison will report in the next section. The output of the backbone network is subsequently fed to a Feature Pyramid Network (FPN) \cite{lin2016feature}. As shown in Fig. \ref{fig:sys_flow} (b), deformable convolution is optionally applied to the downsample layer of FPN which enables an adaptive data sampling on an image. The FPN fuses multiscaled features into a fixed-size feature map where we make a prediction of $s_i$, $s_{\mathcal{N}_i}$ and $\mathbf{P}_i$ for each node with $1\times 1$ convolution window. \par

%In the training phase, the ground-true bounding boxes are converted into node-wise fore/background label $\mathcal{M}_o$ and center label $\mathcal{M}_c$ which are used to compute the $\mathcal{L}_o$, $\mathcal{L}_c$ $g_i$ and $g_{\mathcal{N}_i}$ using Algorithm \ref{alg:train_opt_1}. In the testing phase, we firstly uses the generated fore/background mask $\mathbf{P}$ to remove the background nodes. Then we apply the correlation propagation directly or the Algorithm \ref{alg:gps} to partition nodes to different foreground groups and merge groups whose centers are closed. Finally, all nodes in the foreground groups will be back-project to the original image and the instance-level bounding boxes will be produced by analysis the geometry of projected foreground group with PCA.

\begin{figure}[]
	\centering
	\includegraphics[width=\linewidth]{figures/sys_flow}
	\caption{Work flow of training and inference of Correlation Propagation Networks.}
	\label{fig:sys_flow}
\end{figure}

==> speed.tex <==
\begin{table}[] \renewcommand{\arraystretch}{0.9}
	\centering
	\caption{FPS comparison on ICDAR-13 with input size of $512\times 512$.}
	\label{tab:fps}
	\scalebox{0.9}{
	\begin{tabular}{|l||ccc||c|}
		\hline
		Methods                                                 & P                         & R                                  & F                         & FPS                                \\ \hline
		Yao \cite{yao2012detecting} & 0.63           &0.63       &0.60 &0.14 \\ \hline
		Gupta \cite{gupta2016synthetic} &92.0 &75.5 &83.0 &15 \\ \hline
		TextBox \cite{liao2017textboxes}                      & 0.88                      & 0.83                               & 0.85                      & 20.6                               \\ \hline
		CTPN \cite{tian2016detecting}                         & \textbf{0.93}             & 0.83                               & \textbf{0.88}             & 14.2                               \\ \hline
		SegLink \cite{shi2017detecting}                       & 0.88                      & 0.83                               & 0.85                      & 20.6                               \\ \hline
		\textbf{CPN}                                  & 88.1         & 90.5        & 89.3                      &                             \\ \hline
	\end{tabular}
}
\end{table}
